On the Interplay between Self-Driving Cars and Public Transportation

Cities worldwide struggle with overloaded transportation systems and their externalities. The emerging autonomous transportation technology has the potential to alleviate these issues, but the decisions of profit-maximizing operators running large autonomous fleets could negatively impact other stakeholders and the transportation system. An analysis of these tradeoffs requires modeling the modes of transportation in a unified framework. In this paper, we propose such a framework, which allows us to study the interplay among mobility service providers (MSPs), public transport authorities, and customers. Our framework combines a graph-theoretic network model for the transportation system with a game-theoretic market model in which MSPs are profit maximizers while customers select individually-optimal transportation options. We apply our framework to data for the city of Berlin and present sensitivity analyses to study parameters that MSPs or municipalities can strategically influence. We show that autonomous ride-hailing systems may cannibalize a public transportation system, serving between 7% and 80% of all customers, depending on market conditions and policy restrictions.

==> packages/pgf-pie/demo/before-after-number.tex <==
\begin{tikzpicture}
  \pie[before number={\$}, after number=,]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> packages/pgf-pie/demo/cloud.tex <==
\begin{tikzpicture}
  \pie[cloud, text=inside, scale font]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> packages/pgf-pie/demo/color.tex <==
\begin{tikzpicture}
  \pie[color={black!10, black!20, black!30, black!40}]
  {10/A, 20/B, 30/C, 40/D}

  \pie[pos={8,0}, color=blue!20] {10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}


==> packages/pgf-pie/demo/colorwheel.tex <==
\begin{tikzpicture}
  \pie{10/, 10/, 10/, 10/, 10/, 10/, 10/, 10/, 10/, 10/}
\end{tikzpicture}

==> packages/pgf-pie/demo/explode.tex <==
\begin{tikzpicture}
  % explode list
  \pie[explode={0, 0, 0, 0.1}] {10/A, 20/B, 30/C, 40/D}

  % explode all
  \pie[pos={8,0}, explode=0.1] {10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> packages/pgf-pie/demo/first-pie.tex <==
\begin{tikzpicture}
  \pie{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> packages/pgf-pie/demo/legend.tex <==
\begin{tikzpicture}
  \pie[text=legend]{10/First, 20/Second, 30/Third, 40/Fourth}
\end{tikzpicture}

==> packages/pgf-pie/demo/polar.tex <==
\begin{tikzpicture}
  \pie[polar]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> packages/pgf-pie/demo/population.tex <==
% data from http://en.wikipedia.org/wiki/List_of_countries_by_population
\begin{tikzpicture}
  \pie[cloud, rotate=45, sum=auto, radius=35, after number=, text=pin] {1339/China,
    1210/India, 312/USA, 237/Indonesia, 190/Brazil, 177/Pakistan,
    158/Nigeria, 151/Bangladesh, 142/Russia, 127/Japan, 112/Mexico,
    94/Philippines, 87/Vietnam, 82/Ethiopia, 81/Germany, 80/Egypt,
    75/Iran, 73/Turkey, 67/Thailand, 65/Congo, 65/France, 62/UK,
    60/Italy, 50/South Africa, 48/South Korea, 47/Myanmar, 46/Spain,
    46/Colombia, 45/Ukraine, 43/Tanzania, 40/Argentina, 38/Kenya,
    38/Poland, 36/Algeria, 34/Canada, 32/Morocco, 31/Uganda, 31/Iraq,
    31/Afghanistan, 30/Sudan, 29/Peru, 29/Venezuela, 28/Nepal,
    28/Malaysia, 27/Uzbekistan, 27/Saudi Arabia, 24/Ghana, 24/North
    Korea, 23/Syria, 23/Taiwan, 22/Australia, 22/Yemen, 21/Romania,
    20/Madagascar, 20/Sri Lanka, 20/Mozambique, 19/Cote d'Ivoire,
    19/Cameroon, 19/Angola, 17/Chile, 16/Netherlands, 16/Kazakhstan,
    15/Burkina Faso, 15/Niger, 14/Malawi, 14/Mali, 14/Guatemala,
    14/Ecuador, 13/Cambodia, 13/Zambia, 12/Zimbabwe, 12/Senegal,
    11/Cuba, 11/Chad, 10/Belgium, 10/Greece, 10/Portugal, 10/Tunisia,
    10/Czech Republic, 10/Bolivia, 10/Rwanda, 10/Haiti, 10/Hungary,
    10/Guinea, 10/Belarus, 9/Sweden, 9/Dominican Republic, 9/Somalia,
    9/Azerbaijan, 9/Benin, 8/Austria, 8/Burundi, 8/United Arab
    Emirates, 8/South Sudan, 8/Honduras, 8/Switzerland, 8/Israel,
    7/Bulgaria, 7/Serbia, 7/Hong Kong }

  % \node[circle,draw=black,thick, fill=white, font=\bf]
  % {Population of the world};
\end{tikzpicture}


==> packages/pgf-pie/demo/radius.tex <==
\begin{tikzpicture}
  \pie{10/, 20/, 30/, 40/}

  \pie[pos={8,0}, rotate=180]{10/, 20/, 30/, 40/}

  \pie[pos={17,0}, radius=4]{10/, 20/, 30/, 40/}
\end{tikzpicture}

==> packages/pgf-pie/demo/scalefont.tex <==
\begin{tikzpicture}
  \pie[scale font]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> packages/pgf-pie/demo/shadow.tex <==
% \usetikzlibrary{shadows}
\begin{tikzpicture}
  \pie[style=drop shadow]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}


==> packages/pgf-pie/demo/square.tex <==
\begin{tikzpicture}
  \pie[square]{40/A, 30/B, 20/C, 10/D}
\end{tikzpicture}

==> packages/pgf-pie/demo/sum.tex <==
\begin{tikzpicture}
  \pie[sum=auto, after number=, radius=2]{33/Boys, 7/Girls}

  \pie[pos={6,0}, sum=40, after number=, radius=2]{33/Boys}
\end{tikzpicture}

==> packages/pgf-pie/demo/text-inside.tex <==
\begin{tikzpicture}
  \pie[text=inside]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}

==> packages/pgf-pie/demo/text.tex <==
\begin{tikzpicture}
  \pie[text=pin]{10/A, 20/B, 30/C, 40/D}
\end{tikzpicture}
